MELAC: Massive Evaluation of Large Language Models with Alignment of Culture in Persian Language

As large language models (LLMs) become increasingly embedded in our daily lives, evaluating their quality and reliability across diverse contexts has become essential. While comprehensive benchmarks exist for assessing LLM performance in English, there remains a significant gap in evaluation resources for other languages. Moreover, because most LLMs are trained primarily on data rooted in European and American cultures, they often lack familiarity with non-Western cultural contexts. To address this limitation, our study focuses on the Persian language and Iranian culture. We introduce 19 new evaluation datasets specifically designed to assess LLMs on topics such as Iranian law, Persian grammar, Persian idioms, and university entrance exams. Using these datasets, we benchmarked 41 prominent LLMs, aiming to bridge the existing cultural and linguistic evaluation gap in the field.

==> tables/hyper_prameters_for_evaluation.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c}
    \textbf{Hyperparameter} &  \textbf{Value} \\ \hline
     top\_p &  1.0 \\ \hline
     seed & 1234 \\ \hline
     temperature & 0.0
     \\ 
    \end{tabular}
    \caption{Hyperparameters used for LLM evaluation.}
    \label{tab:evaluation setup}
\end{table}

==> tables/original_datasets.tex <==
\begin{table}[h]
    \centering 
    \def\arraystretch{1.25}
    \setlength{\tabcolsep}{12pt} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|c|c} 
    \hline
    \textbf{Dataset name} & \textbf{Field} &  \textbf{\#  Samples}\\ \hline 
    Iran Rules & Law & 350
    \\ \hline 
    Religious & Religion & 525
    \\ \hline 
    AUT Multiple Choice & Knowledge-based Reasoning & 1000
    \\ \hline 
    Context-based QA (Generation) & Comprehension & 1000
    \\ \hline 
    Context-based QA (Yes/No) & Comprehension & 1000
    \\ \hline
    Persian Literature & Linguistics & 777
    \\ \hline 
    University entrance exam Multiple Choice & Knowledge-based Reasoning & XXXX
    \\ \hline 
    Homographs Easy & Linguistics & 434
    \\ \hline 
    Homographs Hard & Linguistics & 108
    \\ \hline 
    Persian Proverbs & Culture & 370
    \\ \hline 
    Persian Verb Structure (4-Choice) & Linguistics & 1800
    \\ \hline 
    Persian Verb Structure (Generation) & Linguistics & 1500
    \\ \hline 
    General Knowledge & Knowledge & 392
    \\ \hline 
    HellaSwag (Persian adaption) & Reasoning & 500-1000
    \\ \hline 
    \end{tabular}
    }
    \caption{Original datasets that we create in this research.}
    \label{tab:attr}
\end{table}

==> tables/results_table.tex <==
\usepackage{booktabs}

\begin{table*}[h]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrr}
    \toprule
                          Model &  Average &  Arc Challenge New &  Arc Easy New &  Feqh Aut &  Hallucination Hallu &  Hallucination Hallu Y &  Hallucination Right &  Hallucination Right Y &  Hellaswag &  Law Aut &  Multiple Choice New &  Persian Litreture &  Qa Yn Aut &  Reading Qa Aut(Exact) &  Part-Expert &  Mmlu-Pro &  Social Norm &  General Knowledge &  Gsm8K New &  Homograph 2Choice Combined Asterisks &  Homograph 4Choice &  Piqa &  Proverbs &  Verbs &  Winogrande \\
    \midrule
           Qwen2.5-32B-Instruct &    61.68 &              85.15 &         91.87 &     38.86 &                71.00 &                  43.00 &                50.80 &                  76.40 &      82.07 &    42.33 &                50.40 &              40.41 &      93.40 &                   7.70 &        46.78 &     37.40 &        70.00 &              61.73 &      50.10 &                                 67.59 &              91.47 & 83.98 &     63.24 &  54.58 &       80.07 \\
                 gemma-3-27b-it &    61.42 &              88.35 &         94.22 &     24.57 &                37.30 &                  55.40 &                75.00 &                  65.80 &      83.39 &    36.33 &                55.20 &              40.93 &      91.40 &                   1.20 &        49.32 &     36.60 &        70.49 &              73.72 &      28.30 &                                 63.89 &              92.40 & 87.29 &     78.92 &  66.02 &       78.12 \\
                QwQ-32B-Preview &    59.54 &              85.58 &         91.44 &     41.14 &                82.50 &                  97.80 &                25.40 &                   4.10 &      84.13 &    43.00 &                50.60 &              39.77 &      88.50 &                  23.60 &        47.39 &     37.30 &        72.26 &              63.27 &      34.70 &                                 61.11 &              88.25 & 81.28 &     58.11 &  51.97 &       75.64 \\
                 gemma-3-12b-it &    58.91 &              83.33 &         93.26 &     25.14 &                12.40 &                  33.30 &                93.80 &                  74.90 &      83.17 &    36.33 &                49.00 &              40.03 &      87.60 &                   4.50 &        44.12 &     32.60 &        75.55 &              68.37 &      20.20 &                                 67.59 &              91.24 & 87.19 &     72.97 &  63.39 &       73.96 \\
                 gemma-2-27b-it &    58.85 &              86.75 &         94.22 &     24.00 &                 7.00 &                   2.00 &                96.40 &                  99.10 &      83.69 &    34.67 &                50.80 &              35.91 &      89.80 &                   0.10 &        46.60 &     36.90 &        77.38 &              68.11 &      26.70 &                                 60.19 &              91.24 & 89.69 &     73.51 &  61.16 &       76.44 \\
                aya-expanse-32b &    58.81 &              85.15 &         93.37 &     37.14 &                46.50 &                   8.60 &                43.30 &                  79.20 &      81.70 &    38.67 &                54.70 &              34.75 &      89.70 &                  24.90 &        44.29 &     32.10 &        74.94 &              73.72 &      17.50 &                                 62.96 &              87.56 & 91.19 &     77.03 &  61.95 &       70.50 \\
                        QwQ-32B &    58.64 &              84.94 &         90.80 &     41.71 &                76.80 &                   7.50 &                35.90 &                  97.00 &      82.22 &    38.00 &                49.30 &              37.71 &      88.50 &                  17.80 &        46.73 &     39.00 &        70.73 &              60.71 &      29.30 &                                 58.33 &              88.25 & 81.68 &     59.19 &  52.31 &       73.07 \\
                      Qwen3-14B &    56.82 &              84.29 &         91.02 &     29.14 &                96.10 &                  77.80 &                 9.80 &                  31.20 &      80.97 &    34.67 &                44.80 &              35.39 &      87.60 &                  24.40 &        43.22 &     35.50 &        74.51 &              56.38 &      31.10 &                                 55.56 &              87.56 & 77.18 &     53.78 &  54.36 &       67.32 \\
                  gemma-2-9b-it &    56.76 &              84.29 &         93.16 &     29.71 &                38.40 &                  49.50 &                56.70 &                  51.70 &      80.82 &    33.67 &                48.50 &              38.10 &      89.70 &                   0.10 &        43.03 &     33.20 &        73.84 &              64.03 &      17.40 &                                 59.26 &              90.55 & 87.09 &     69.19 &  58.25 &       72.01 \\
                     aya-23-35B &    54.15 &              77.56 &         90.16 &     30.29 &                84.10 &                   1.00 &                 6.30 &                  99.10 &      79.87 &    32.00 &                48.70 &              31.92 &      86.20 &                  23.70 &        37.44 &     24.10 &        65.00 &              63.27 &      10.00 &                                 55.56 &              83.64 & 89.49 &     67.03 &  47.32 &       65.81 \\
                       Qwen3-8B &    52.86 &              80.24 &         87.38 &     28.00 &                15.10 &                  70.10 &                81.40 &                  26.50 &      80.38 &    29.67 &                46.00 &              33.20 &      86.40 &                  25.00 &        38.31 &     31.10 &        63.41 &              49.23 &      25.70 &                                 50.93 &              82.95 & 75.98 &     51.89 &  47.93 &       61.91 \\
                 aya-expanse-8b &    52.29 &              71.47 &         84.60 &     29.71 &                13.80 &                  12.30 &                79.50 &                  89.70 &      76.49 &    32.33 &                45.80 &              34.49 &      82.30 &                  20.10 &        35.56 &     21.90 &        71.71 &              58.67 &       9.80 &                                 51.85 &              80.65 & 80.18 &     60.00 &  48.06 &       64.04 \\
                      Hormoz-8B &    51.79 &              70.41 &         84.28 &     28.57 &                13.90 &                   7.50 &                79.50 &                  92.40 &      76.05 &    30.33 &                46.70 &              33.08 &      79.80 &                  19.60 &        36.46 &     21.50 &        70.30 &              58.42 &      10.00 &                                 50.93 &              80.65 & 80.68 &     60.27 &  47.29 &       64.39 \\
          Llama-3.1-8B-Instruct &    50.70 &              68.91 &         80.11 &     29.71 &                 3.20 &                   3.50 &                99.20 &                  99.20 &      79.79 &    32.67 &                44.90 &              32.30 &      82.70 &                  24.50 &        37.62 &     25.70 &        70.98 &              52.55 &      12.00 &                                 43.52 &              79.03 & 70.07 &     47.57 &  42.91 &       54.21 \\
            Qwen2.5-7B-Instruct &    50.27 &              72.33 &         81.50 &     36.57 &                19.90 &                  24.10 &                73.10 &                  63.20 &      74.80 &    32.33 &                42.60 &              31.27 &      82.50 &                  17.60 &        37.24 &     26.70 &        64.51 &              51.02 &      18.00 &                                 52.78 &              79.26 & 71.07 &     47.84 &  44.44 &       61.91 \\
                      aya-23-8B &    49.21 &              63.68 &         81.39 &     29.14 &               100.00 &                  99.60 &                 0.00 &                   0.30 &      75.83 &    28.33 &                42.90 &              31.27 &      72.30 &                  23.40 &        33.33 &     19.90 &        70.73 &              52.30 &       6.10 &                                 52.78 &              76.27 & 80.78 &     44.32 &  39.30 &       57.13 \\
       c4ai-command-r7b-12-2024 &    49.01 &              68.70 &         81.18 &     26.29 &                71.80 &                   7.30 &                30.90 &                  89.30 &      72.89 &    31.67 &                44.70 &              32.18 &      67.50 &                  21.00 &        35.92 &     22.90 &        56.40 &              52.55 &      10.10 &                                 47.22 &              71.43 & 75.88 &     56.76 &  42.45 &       59.17 \\
              Qwen2-7B-Instruct &    48.97 &              69.12 &         80.75 &     28.00 &                76.80 &                  86.50 &                15.60 &                  12.30 &      76.71 &    28.33 &                40.40 &              31.40 &      79.00 &                  10.90 &        36.31 &     23.80 &        62.20 &              52.04 &      14.50 &                                 54.63 &              72.81 & 70.97 &     50.54 &  40.62 &       60.94 \\
       Meta-Llama-3-8B-Instruct &    48.25 &              66.77 &         76.47 &     33.71 &                 0.70 &                  44.00 &                96.70 &                  26.70 &      76.71 &    32.00 &                45.00 &              29.99 &      82.50 &                  19.40 &        36.30 &     26.00 &        70.06 &              52.04 &      10.40 &                                 41.67 &              81.11 & 70.97 &     42.97 &  38.93 &       56.95 \\
                  gemma-3-4b-it &    48.13 &              63.46 &         79.57 &     21.14 &                74.80 &                  33.60 &                30.40 &                  73.10 &      73.84 &    27.67 &                42.50 &              30.24 &      78.60 &                   5.50 &        34.70 &     22.80 &        65.55 &              45.92 &       9.60 &                                 42.59 &              72.58 & 72.77 &     53.78 &  45.30 &       55.09 \\
                       Qwen3-4B &    48.03 &              73.61 &         83.42 &     30.29 &                60.30 &                  72.80 &                16.00 &                  11.00 &      78.03 &    30.33 &                40.60 &              31.79 &      81.90 &                  21.30 &        37.28 &     28.90 &        68.72 &              43.88 &      20.10 &                                 38.89 &              76.27 & 66.07 &     45.41 &  41.23 &       54.56 \\
          Hermes-3-Llama-3.1-8B &    47.88 &              65.28 &         78.07 &     30.29 &                40.90 &                  29.00 &                50.50 &                  59.00 &      73.99 &    31.67 &                42.10 &              30.63 &      83.50 &                  13.50 &        35.61 &     24.10 &        54.88 &              49.49 &      10.20 &                                 44.44 &              79.72 & 70.37 &     47.84 &  48.94 &       55.18 \\
    Dorna2-Llama3.1-8B-Instruct &    47.84 &              67.63 &         78.72 &     33.71 &                22.50 &                   1.10 &                68.80 &                  99.20 &      78.91 &    29.67 &                41.00 &              27.28 &      81.80 &                  21.90 &        36.16 &     22.70 &        49.82 &              48.72 &      11.90 &                                 44.44 &              72.81 & 69.97 &     42.97 &  42.06 &       54.47 \\
                   Llama-3.1-8B &    46.73 &              63.35 &         75.08 &     30.86 &                73.00 &                  39.30 &                20.90 &                  52.70 &      76.34 &    33.00 &                42.60 &              27.41 &      71.60 &                  19.70 &        35.92 &     22.20 &        61.83 &              49.23 &      10.80 &                                 46.30 &              72.12 & 66.47 &     35.95 &  39.91 &       54.92 \\
                Meta-Llama-3-8B &    46.53 &              62.07 &         75.83 &     27.43 &                91.10 &                  25.50 &                 7.50 &                  67.40 &      76.49 &    35.67 &                42.50 &              28.19 &      75.20 &                  19.50 &        35.10 &     22.80 &        54.02 &              47.70 &      10.30 &                                 41.67 &              74.42 & 64.16 &     37.30 &  39.46 &       55.36 \\
       Dorna-Llama3-8B-Instruct &    44.78 &              59.94 &         70.70 &     29.14 &                71.50 &                  22.60 &                16.20 &                  51.90 &      75.68 &    25.33 &                36.90 &              27.54 &      80.10 &                  21.80 &        34.49 &     22.00 &        69.39 &              41.33 &      10.30 &                                 40.74 &              74.65 & 66.17 &     35.41 &  34.74 &       56.16 \\
                  gemma-2-2b-it &    43.08 &              57.91 &         70.48 &     25.71 &                28.60 &                  18.30 &                61.40 &                  74.30 &      69.88 &    32.67 &                36.90 &              30.76 &      72.40 &                   0.30 &        31.31 &     18.20 &        40.18 &              32.91 &       6.40 &                                 47.22 &              74.65 & 66.87 &     45.68 &  36.18 &       54.74 \\
                  gemma-3-1b-it &    38.55 &              36.43 &         46.10 &     28.00 &                56.80 &                  80.10 &                53.20 &                  32.80 &      63.92 &    20.33 &                29.10 &              24.97 &      63.90 &                   2.10 &        27.22 &     13.70 &        51.22 &              26.02 &       4.30 &                                 49.07 &              51.15 & 57.66 &     28.92 &  27.67 &       50.58 \\
          Llama-3.2-1B-Instruct &    37.43 &              37.50 &         47.38 &     31.43 &                 1.70 &                   0.00 &                95.80 &                 100.00 &      55.40 &    24.00 &                29.90 &              27.03 &      64.10 &                   7.20 &        28.59 &     15.70 &        37.44 &              29.59 &       4.10 &                                 50.93 &              52.53 & 54.05 &     28.65 &  26.11 &       49.07 \\
               Maral-7B-alpha-1 &    36.23 &              37.29 &         43.10 &     26.29 &               100.00 &                   0.00 &                 0.00 &                 100.00 &      60.18 &    26.33 &                28.40 &              26.77 &      62.70 &                  10.80 &        27.10 &     14.80 &        24.63 &              31.63 &       6.10 &                                 43.52 &              47.47 & 51.95 &     22.16 &  28.96 &       49.42 \\
                   Llama-3.2-1B &    33.23 &              28.63 &         32.94 &     22.29 &                99.70 &                   0.20 &                 0.60 &                 100.00 &      39.60 &    22.00 &                27.20 &              25.23 &      63.80 &                   5.90 &        26.16 &     13.70 &        25.06 &              25.26 &       2.40 &                                 57.41 &              27.42 & 49.65 &     26.76 &  26.45 &       49.25 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Benchmark results over 34 LLMs.}
    \label{tab:your_table_label}
\end{table*}

==> tables/translation_vs_localization.tex <==
% \begin{table}[h]
%     \centering 
%     \def\arraystretch{1.05} % Increased for more vertical spacing
%     \setlength{\tabcolsep}{9pt} 
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{|p{0.3\linewidth}|p{0.7\linewidth}|} % Adjusted column width
%     \hline
%     \textbf{Original Question} & In {\color{red} 1872}, the  {\color{red}United States} created a national park called {\color{red}Yellowstone}. The park includes more than two million acres in the three states of   {\color{red}Idaho}, {\color{red}Montana}, and {\color{red}Wyoming}. Which statement best explains why national parks have a positive effect on ecosystems? \\ \hline 
%     \textbf{Translated Question} & 
%     \foreignlanguage{arabic}{
%     \begin{flushright}
%     \begin{RTL}{
% در سال {\color{blue}{۱۸۷۲}}، {\color{blue}ایالات متحده} یک پارک ملی به نام {\color{blue}{یلوستون}} ایجاد کرد. این پارک بیش از {\color{blue}{دو میلیون}} هکتار را در سه ایالت {\color{blue}آیداهو}، {\color{blue}مونتانا}، و {\color{blue}وایومینگ} شامل می‌شود. کدام گزاره به بهترین شکل توضیح می‌دهد که چرا پارک‌های ملی تأثیر مثبتی بر اکوسیستم‌ها دارند؟
% }\end{RTL}
% \end{flushright}
% }


%     \\ \hline 
%     \textbf{Translated + Localized Question} & 
%         \begin{flushright}
%     \foreignlanguage{arabic}{
% در سال {\color{ForestGreen}{۱۳۵۱}}، {\color{ForestGreen}{ایران}} یک پارک ملی به نام {\color{ForestGreen}{پارک ملی}} {\color{ForestGreen}{گلستان}} ایجاد کرد. این پارک بیش از {\color{ForestGreen}{۹۱ هزار}} هکتار را در استان‌های {\color{ForestGreen}{گلستان}}، {\color{ForestGreen}{خراسان شمالی}} و {\color{ForestGreen}{سمنان}} در بر می‌گیرد. کدام گزینه بهترین توضیح را درباره اینکه چرا پارک‌های ملی تأثیر مثبتی بر اکوسیستم‌ها دارند، ارائه می‌دهد؟
% }




% \end{flushright}
%     \\ \hline 
%     \end{tabular}
%     }
%     \caption{Comparison of direct translation versus culturally-adapted (localized) translation, illustrating proper noun and name adaptations for the Persian context. The blue color denotes the identified localization targets, and the green color marks the Persian equivalents used for those targets. The Persian equivalents are not exact matches; they have been selected to fit the same context.}
%     \label{tab:attr}
% \end{table}

==> tables/uncertaintyWOhallu.tex <==


\begin{table*}[h]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Model &  Average &  Feqh &  Law &  MC &  PL &  QA YN &  Expert &  SN &  Hellaswag &  GK &  Hh &  He &  Proverbs &  Verbs \\
\hline
Llama-3.1-8B             &     \textcolor{purple}{0.86} &      \textcolor{purple}{0.96} &     \textcolor{purple}{0.94} &                 0.89 &               \textcolor{purple}{0.95} &       0.91 &         0.92 &         0.98 &       0.66 &               0.83 &                                  0.80 &               0.54 &      0.89 &   0.94 \\
Maral-7B-alpha-1         &     \textcolor{purple}{0.86} &      0.92 &     0.93 &                 0.89 &               0.91 &       0.88 &         0.90 &         0.89 &       0.78 &               0.87 &                                  \textcolor{purple}{0.83} &               \textcolor{purple}{0.75} &      \textcolor{purple}{0.92} &   0.86 \\
Meta-Llama-3-8B          &     0.85 &      \textcolor{purple}{0.96} &     \textcolor{purple}{0.94} &                 0.86 &               \textcolor{purple}{0.95} &      \textcolor{purple}{ 0.92} &         0.91 &         \textcolor{purple}{0.99} &       0.64 &               0.77 &                                  0.80 &               0.49 &      0.87 &   0.92 \\
PersianMind-v1           &     0.82 &      0.95 &     0.93 &                 \textcolor{purple}{0.94} &               0.94 &       \textcolor{purple}{0.92} &         \textcolor{purple}{0.93} &         0.94 &       \textcolor{purple}{0.86} &               \textcolor{purple}{0.89} &                                  0.74 &               0.73 &      0.88 &   \textcolor{purple}{0.96} \\
Llama-3.2-1B-Instruct    &     0.74 &      0.83 &     0.79 &                 0.77 &               0.80 &       0.33 &         0.78 &         0.75 &       0.80 &               0.75 &                                  0.63 &               0.61 &      0.72 &   0.70 \\
Dorna-Llama3-8B-Instruct &     0.69 &      0.83 &     0.74 &                 0.75 &               0.80 &       0.48 &         0.77 &         0.84 &       0.39 &               0.65 &                                  0.64 &               0.32 &      0.70 &   0.73 \\
aya-23-8B                &     0.67 &      0.88 &     0.81 &                 0.75 &               0.85 &       0.52 &         0.79 &         0.83 &       0.51 &               0.59 &                                  0.46 &               0.29 &      0.72 &   0.68 \\
Llama-3.1-8B-Instruct    &     0.62 &      0.90 &     0.84 &                 0.76 &               0.84 &       0.60 &         0.80 &         0.81 &       0.40 &               0.60 &                                  0.60 &               0.23 &      0.68 &   0.81 \\
Qwen3-14B                &     0.61 &      0.75 &     0.73 &                 0.66 &               0.75 &       0.31 &         0.66 &         0.67 &       0.39 &               0.51 &                                  0.70 &               0.24 &      0.61 &   0.65 \\
Qwen3-8B                 &     0.55 &      0.80 &     0.69 &                 0.63 &               0.76 &       0.21 &         0.57 &         0.67 &       0.29 &               0.48 &                                  0.40 &               0.17 &      0.62 &   0.69 \\
Meta-Llama-3-8B-Instruct &     0.55 &      0.73 &     0.60 &                 0.62 &               0.67 &       0.31 &         0.66 &         0.53 &       0.20 &               0.44 &                                  0.50 &               0.13 &      0.51 &   0.54 \\
Qwen3-32B                &     0.53 &      0.75 &     0.71 &                 0.75 &               0.73 &       0.25 &         0.58 &         0.48 &       0.32 &               0.52 &                                  0.63 &               0.21 &      0.43 &   0.53 \\
QwQ-32B-Preview          &     0.52 &      0.70 &     0.64 &                 0.60 &               0.67 &       0.36 &         0.62 &         0.60 &       0.21 &               0.43 &                                  0.50 &               0.19 &      0.45 &   0.61 \\
QwQ-32B                  &     0.52 &      0.66 &     0.67 &                 0.62 &               0.68 &       0.36 &         0.63 &         0.56 &       0.25 &               0.45 &                                  0.60 &               0.18 &      0.45 &   0.62 \\
Qwen3-4B                 &     0.49 &      0.54 &     0.48 &                 0.56 &               0.60 &       0.22 &         0.54 &         0.72 &       0.23 &               0.39 &                                  0.43 &               0.16 &      0.48 &   0.49 \\
aya-23-35B               &     0.48 &      0.61 &     0.57 &                 0.48 &               0.66 &       0.20 &         0.55 &         0.63 &       0.15 &               0.29 &                                  0.40 &               0.13 &      0.35 &   0.51 \\
gemma-2-2b-it            &     0.47 &      0.57 &     0.59 &                 0.52 &               0.61 &       0.10 &         0.47 &         0.24 &       0.32 &               0.44 &                                  0.10 &               0.07 &      0.40 &   0.41 \\
Qwen3-30B-A3B            &     0.46 &      0.77 &     0.71 &                 0.57 &               0.71 &       0.29 &         0.54 &         0.61 &       0.24 &               0.42 &                                  0.50 &               0.13 &      0.37 &   0.46 \\
gemma-3-1b-it            &     0.40 &      0.55 &     0.46 &                 0.44 &               0.53 &       0.08 &         0.56 &         \textcolor{violet}{0.04} &       0.40 &               0.38 &                                  0.11 &               0.21 &      0.23 &   0.27 \\
Qwen2-7B-Instruct        &     0.33 &      0.44 &     0.33 &                 0.30 &               0.39 &       0.18 &         0.37 &         0.36 &       0.09 &               0.23 &                                  0.11 &               0.07 &      0.18 &   0.30 \\
Qwen2.5-7B-Instruct      &     0.32 &      0.55 &     0.51 &                 0.40 &               0.51 &       0.20 &         0.42 &         0.35 &       0.08 &               0.28 &                                  0.17 &               0.06 &      0.19 &   0.28 \\
gemma-2-9b-it            &     0.31 &      0.57 &     0.40 &                 0.45 &               0.47 &       0.07 &         0.38 &         0.08 &       0.09 &               0.22 &                                  0.19 &              \textcolor{violet}{0.02} &      0.17 &   0.28 \\
aya-expanse-32b          &     0.30 &      0.53 &     0.45 &                 0.42 &               0.46 &       0.08 &         0.40 &         0.24 &       0.06 &               0.19 &                                  0.16 &               0.04 &      0.09 &   0.32 \\
Qwen2.5-32B-Instruct     &     0.30 &      0.41 &     0.36 &                 0.41 &               0.39 &       0.07 &         0.37 &         0.21 &       0.12 &               0.21 &                                  0.24 &               0.09 &      0.20 &   0.41 \\
Hormoz-8B                &     0.23 &      0.44 &     0.37 &                 0.32 &               0.38 &       0.32 &         0.36 &         0.19 &       0.06 &               0.20 &                                  0.15 &               0.03 &      0.11 &   0.27 \\
aya-expanse-8b           &     0.23 &      0.46 &     0.36 &                 0.32 &               0.40 &       0.30 &         0.34 &         0.17 &       0.06 &               0.21 &                                  0.16 &               0.03 &      0.13 &   0.27 \\
gemma-3-4b-it            &     0.22 &      0.33 &     0.20 &                 0.24 &               0.36 &       0.06 &         0.25 &         0.12 &       0.08 &               0.10 &                                  0.07 &               0.03 &      0.10 &   0.19 \\
gemma-2-27b-it           &     0.21 &      0.38 &     0.28 &                 0.37 &               0.33 &       0.05 &         0.28 &         0.09 &       0.04 &               0.15 &                                  0.09 &               \textcolor{violet}{0.02} &      0.09 &   0.22 \\
gemma-3-27b-it           &     0.19 &      0.25 &     0.15 &                 0.23 &               \textcolor{violet}{0.20} &  \textcolor{violet}{0.02} &         \textcolor{violet}{0.18} &         0.11 &       \textcolor{violet}{0.03} &               \textcolor{violet}{0.06} &                                  0.17 &               \textcolor{violet}{0.02} &      0.05 &   \textcolor{violet}{0.10} \\
gemma-3-12b-it           &     \textcolor{violet}{0.16} &      \textcolor{violet}{0.19} &     \textcolor{violet}{0.14} &                 \textcolor{violet}{0.21} &               0.26 &       \textcolor{violet}{0.02} &         \textcolor{violet}{0.18} &         \textcolor{violet}{0.04} &       \textcolor{violet}{0.03} &               0.09 &                                  \textcolor{violet}{0.06} &               \textcolor{violet}{0.02} &      \textcolor{violet}{0.04} &   0.16 \\ \hline
\bottomrule
\end{tabular}




    }
    \caption{uncertainty of LLMs on multiple choice Original datasets not containing hallucination sorted by average performance.}
    \label{tab:uncertainty-original-wo-hallu}
\end{table*}

==> tables/uncertainty_original.tex <==
% \usepackage{booktabs}

\begin{table*}[h]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Model &  Average &  Feqh &  Law &  MC &  PL &  QA YN &  Expert &  SN &  Hellaswag &  GK &  Hh &  He &  Proverbs &  Verbs &  Hallu &  Hallu Right \\
\hline
Llama-3.1-8B             &     0.86 &      0.96 &     0.94 &                 0.89 &               0.95 &       0.91 &         0.92 &         0.98 &       0.66 &               0.83 &                                  0.80 &               0.54 &      0.89 &   0.94 &                 0.62 &                 0.99 \\
Maral-7B-alpha-1         &     0.86 &      0.92 &     0.93 &                 0.89 &               0.91 &       0.88 &         0.90 &         0.89 &       0.78 &               0.87 &                                  0.83 &               0.75 &      0.92 &   0.86 &                 0.51 &                 0.78 \\
Meta-Llama-3-8B          &     0.85 &      0.96 &     0.94 &                 0.86 &               0.95 &       0.92 &         0.91 &         0.99 &       0.64 &               0.77 &                                  0.80 &               0.49 &      0.87 &   0.92 &                 0.62 &                 0.98 \\
PersianMind-v1           &     0.82 &      0.95 &     0.93 &                 0.94 &               0.94 &       0.92 &         0.93 &         0.94 &       0.86 &               0.89 &                                  0.74 &               0.73 &      0.88 &   0.96 &                 0.21 &                 0.34 \\
Llama-3.2-1B-Instruct    &     0.74 &      0.83 &     0.79 &                 0.77 &               0.80 &       0.33 &         0.78 &         0.75 &       0.80 &               0.75 &                                  0.63 &               0.61 &      0.72 &   0.70 &                 0.60 &                 0.95 \\
Dorna-Llama3-8B-Instruct &     0.69 &      0.83 &     0.74 &                 0.75 &               0.80 &       0.48 &         0.77 &         0.84 &       0.39 &               0.65 &                                  0.64 &               0.32 &      0.70 &   0.73 &                 0.62 &                 0.96 \\
aya-23-8B                &     0.67 &      0.88 &     0.81 &                 0.75 &               0.85 &       0.52 &         0.79 &         0.83 &       0.51 &               0.59 &                                  0.46 &               0.29 &      0.72 &   0.68 &                 0.51 &                 0.81 \\
Llama-3.1-8B-Instruct    &     0.62 &      0.90 &     0.84 &                 0.76 &               0.84 &       0.60 &         0.80 &         0.81 &       0.40 &               0.60 &                                  0.60 &               0.23 &      0.68 &   0.81 &                 0.43 &                 0.69 \\
Qwen3-14B                &     0.61 &      0.75 &     0.73 &                 0.66 &               0.75 &       0.31 &         0.66 &         0.67 &       0.39 &               0.51 &                                  0.70 &               0.24 &      0.61 &   0.65 &                 0.49 &                 0.83 \\
Qwen3-8B                 &     0.55 &      0.80 &     0.69 &                 0.63 &               0.76 &       0.21 &         0.57 &         0.67 &       0.29 &               0.48 &                                  0.40 &               0.17 &      0.62 &   0.69 &                 0.44 &                 0.76 \\
Meta-Llama-3-8B-Instruct &     0.55 &      0.73 &     0.60 &                 0.62 &               0.67 &       0.31 &         0.66 &         0.53 &       0.20 &               0.44 &                                  0.50 &               0.13 &      0.51 &   0.54 &                 0.51 &                 0.88 \\
Qwen3-32B                &     0.53 &      0.75 &     0.71 &                 0.75 &               0.73 &       0.25 &         0.58 &         0.48 &       0.32 &               0.52 &                                  0.63 &               0.21 &      0.43 &   0.53 &                 0.50 &                 0.77 \\
QwQ-32B-Preview          &     0.52 &      0.70 &     0.64 &                 0.60 &               0.67 &       0.36 &         0.62 &         0.60 &       0.21 &               0.43 &                                  0.50 &               0.19 &      0.45 &   0.61 &                 0.49 &                 0.87 \\
QwQ-32B                  &     0.52 &      0.66 &     0.67 &                 0.62 &               0.68 &       0.36 &         0.63 &         0.56 &       0.25 &               0.45 &                                  0.60 &               0.18 &      0.45 &   0.62 &                 0.43 &                 0.75 \\
Qwen3-4B                 &     0.49 &      0.54 &     0.48 &                 0.56 &               0.60 &       0.22 &         0.54 &         0.72 &       0.23 &               0.39 &                                  0.43 &               0.16 &      0.48 &   0.49 &                 0.53 &                 0.80 \\
aya-23-35B               &     0.48 &      0.61 &     0.57 &                 0.48 &               0.66 &       0.20 &         0.55 &         0.63 &       0.15 &               0.29 &                                  0.40 &               0.13 &      0.35 &   0.51 &                 0.55 &                 0.89 \\
gemma-2-2b-it            &     0.47 &      0.57 &     0.59 &                 0.52 &               0.61 &       0.10 &         0.47 &         0.24 &       0.32 &               0.44 &                                  0.10 &               0.07 &      0.40 &   0.41 &                 0.60 &                 0.96 \\
Qwen3-30B-A3B            &     0.46 &      0.77 &     0.71 &                 0.57 &               0.71 &       0.29 &         0.54 &         0.61 &       0.24 &               0.42 &                                  0.50 &               0.13 &      0.37 &   0.46 &                 0.51 &                 0.76 \\
gemma-3-1b-it            &     0.40 &      0.55 &     0.46 &                 0.44 &               0.53 &       0.08 &         0.56 &         0.04 &       0.40 &               0.38 &                                  0.11 &               0.21 &      0.23 &   0.27 &                 0.47 &                 0.71 \\
Qwen2-7B-Instruct        &     0.33 &      0.44 &     0.33 &                 0.30 &               0.39 &       0.18 &         0.37 &         0.36 &       0.09 &               0.23 &                                  0.11 &               0.07 &      0.18 &   0.30 &                 0.51 &                 0.80 \\
Qwen2.5-7B-Instruct      &     0.32 &      0.55 &     0.51 &                 0.40 &               0.51 &       0.20 &         0.42 &         0.35 &       0.08 &               0.28 &                                  0.17 &               0.06 &      0.19 &   0.28 &                 0.18 &                 0.37 \\
gemma-2-9b-it            &     0.31 &      0.57 &     0.40 &                 0.45 &               0.47 &       0.07 &         0.38 &         0.08 &       0.09 &               0.22 &                                  0.19 &               0.02 &      0.17 &   0.28 &                 0.41 &                 0.74 \\
aya-expanse-32b          &     0.30 &      0.53 &     0.45 &                 0.42 &               0.46 &       0.08 &         0.40 &         0.24 &       0.06 &               0.19 &                                  0.16 &               0.04 &      0.09 &   0.32 &                 0.44 &                 0.65 \\
Qwen2.5-32B-Instruct     &     0.30 &      0.41 &     0.36 &                 0.41 &               0.39 &       0.07 &         0.37 &         0.21 &       0.12 &               0.21 &                                  0.24 &               0.09 &      0.20 &   0.41 &                 0.26 &                 0.48 \\
Hormoz-8B                &     0.23 &      0.44 &     0.37 &                 0.32 &               0.38 &       0.32 &         0.36 &         0.19 &       0.06 &               0.20 &                                  0.15 &               0.03 &      0.11 &   0.27 &                 0.23 &                 0.40 \\
aya-expanse-8b           &     0.23 &      0.46 &     0.36 &                 0.32 &               0.40 &       0.30 &         0.34 &         0.17 &       0.06 &               0.21 &                                  0.16 &               0.03 &      0.13 &   0.27 &                 0.20 &                 0.36 \\
gemma-3-4b-it            &     0.22 &      0.33 &     0.20 &                 0.24 &               0.36 &       0.06 &         0.25 &         0.12 &       0.08 &               0.10 &                                  0.07 &               0.03 &      0.10 &   0.19 &                 0.35 &                 0.62 \\
gemma-2-27b-it           &     0.21 &      0.38 &     0.28 &                 0.37 &               0.33 &       0.05 &         0.28 &         0.09 &       0.04 &               0.15 &                                  0.09 &               0.02 &      0.09 &   0.22 &                 0.27 &                 0.42 \\
gemma-3-27b-it           &     0.19 &      0.25 &     0.15 &                 0.23 &               0.20 &       0.02 &         0.18 &         0.11 &       0.03 &               0.06 &                                  0.17 &               0.02 &      0.05 &   0.10 &                 0.41 &                 0.63 \\
gemma-3-12b-it           &     0.16 &      0.19 &     0.14 &                 0.21 &               0.26 &       0.02 &         0.18 &         0.04 &       0.03 &               0.09 &                                  0.06 &               0.02 &      0.04 &   0.16 &                 0.17 &                 0.20 \\ \hline
\bottomrule
\end{tabular}




    }
    \caption{uncertainty of LLMs on multiple choice Original datasets sorted by average performance.}
    \label{tab:uncertainty original}
\end{table*}

==> tables/uncertainty_trans_loc.tex <==
% \usepackage{booktabs}

\begin{table*}[h]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Model &  Average &  Arc Challenge &  Arc Easy &  MMLU-Pro &  PIQA &  Winogrande \\

\hline
Llama-3.1-8B             &     \biggestnumber{0.86} &               0.75 &          0.65 &      \biggestnumber{0.88} &  0.91 &            \biggestnumber{0.98} \\
Maral-7B-alpha-1         &     \biggestnumber{0.86} &               \biggestnumber{0.88} &          \biggestnumber{0.86 }&      \biggestnumber{0.88} &  0.85 &            0.87 \\
Meta-Llama-3-8B          &     0.85 &               0.75 &          0.64 &      0.87 &  \biggestnumber{0.92} &            0.97 \\
PersianMind-v1           &     0.82 &               0.82 &          0.72 &      0.74 &  0.91 &            0.94 \\
Llama-3.2-1B-Instruct    &     0.74 &               0.74 &          0.69 &      0.76 &  0.88 &            0.84 \\
Dorna-Llama3-8B-Instruct &     0.69 &               0.51 &          0.44 &      0.65 &  0.65 &            0.83 \\
aya-23-8B                &     0.67 &               0.53 &          0.37 &      0.79 &  0.56 &            0.78 \\
Llama-3.1-8B-Instruct    &     0.62 &               0.49 &          0.37 &      0.75 &  0.68 &            0.81 \\
Qwen3-14B                &     0.61 &               0.32 &          0.24 &      0.63 &  0.67 &            0.77 \\
Qwen3-8B                 &     0.55 &               0.22 &          0.17 &      0.54 &  0.55 &            0.54 \\
Meta-Llama-3-8B-Instruct &     0.55 &               0.32 &          0.24 &      0.56 &  0.53 &            0.79 \\
Qwen3-32B                &     0.53 &               0.29 &          0.25 &      0.54 &  0.46 &            0.67 \\
QwQ-32B-Preview          &     0.52 &               0.22 &          0.18 &      0.51 &  0.43 &            0.68 \\
QwQ-32B                  &     0.52 &               0.29 &          0.24 &      0.60 &  0.52 &            0.76 \\
Qwen3-4B                 &     0.49 &               0.16 &          0.11 &      0.44 &  0.57 &            0.37 \\
aya-23-35B               &     0.48 &               0.18 &          0.11 &      0.67 &  0.24 &            0.50 \\
gemma-2-2b-it            &     0.47 &               0.34 &          0.24 &      0.70 &  0.43 &            0.65 \\
Qwen3-30B-A3B            &     0.46 &               0.20 &          0.13 &      0.55 &  0.51 &            0.69 \\
gemma-3-1b-it            &     0.40 &               0.53 &          0.46 &      0.66 &  0.33 &            0.37 \\
Qwen2-7B-Instruct        &     0.33 &               0.15 &          0.09 &      0.35 &  0.16 &            0.22 \\
Qwen2.5-7B-Instruct      &     0.32 &               0.19 &          0.13 &      0.44 &  0.21 &            0.27 \\
gemma-2-9b-it            &     0.31 &               0.08 &          0.05 &      0.41 &  0.24 &            0.34 \\
aya-expanse-32b          &     0.30 &               0.10 &          0.06 &      0.40 &  0.14 &            0.39 \\
Qwen2.5-32B-Instruct     &     0.30 &               0.12 &          0.09 &      0.35 &  0.18 &            0.27 \\
Hormoz-8B                &     0.23 &               0.12 &          0.08 &      0.37 &  0.10 &            0.33 \\
aya-expanse-8b           &     0.23 &               0.13 &          0.08 &      0.38 &  0.12 &            0.34 \\
gemma-3-4b-it            &     0.22 &               0.08 &          0.06 &      0.37 &  0.17 &            \textcolor{violet}{0.18} \\
gemma-2-27b-it           &     0.21 &               0.04 &          0.02 &      0.30 &  0.13 &            0.26 \\
gemma-3-27b-it           &     0.19 &              \textcolor{violet}{ 0.03} &          0.01 &      \textcolor{violet}{0.15} &  0.10 &            \textcolor{violet}{0.18} \\
gemma-3-12b-it           &     \textcolor{violet}{0.16} &               0.04 &          0.03 &      0.21 &  \textcolor{violet}{0.08} &            \textcolor{violet}{0.18} \\
\hline
\bottomrule
\end{tabular}




    }
    \caption{uncertainty of LLMs on multiple choice translated/localized datasets sorted by average performance.}
    \label{tab:uncertainty-trans-loc}
\end{table*}
